Toward Fully Autonomous Driving: AI, Challenges, Opportunities, and Needs

Automated driving (AD) is promising, but the transition to fully autonomous driving is, among other things, subject to the real, ever-changing open world and the resulting challenges. However, research in the field of AD demonstrates the ability of artificial intelligence (AI) to outperform classical approaches, handle higher complexities, and reach a new level of autonomy. At the same time, the use of AI raises further questions of safety and transferability. To identify the challenges and opportunities arising from AI concerning autonomous driving functionalities, we have analyzed the current state of AD, outlined limitations, and identified foreseeable technological possibilities. Thereby, various further challenges are examined in the context of prospective developments. In this way, this article reconsiders fully autonomous driving with respect to advancements in the field of AI and carves out the respective needs and resulting research questions.

==> settings/commands.tex <==
\title{Towards Fully Autonomous Driving: \\AI, Challenges, Opportunities, and Needs}

\author{Lars Ullrich\IEEEauthorrefmark{2} \orcidicon{0009-0001-8166-3118} , Michael Buchholz\IEEEauthorrefmark{3} \orcidicon{0000-0001-5973-0794} , Klaus Dietmayer\IEEEauthorrefmark{3} \orcidicon{0000-0002-1651-014X} ,~\IEEEmembership{Senior Member,~IEEE,} \\and Knut Graichen\IEEEauthorrefmark{2} \orcidicon{0000-0003-2865-8093} ,~\IEEEmembership{Senior Member,~IEEE}
	% <-this % stops a space
	\thanks{This research is accomplished within the project ”AUTOtech.agil” (FKZ 01IS22088Y, FKZ 01IS22088W). We acknowledge the financial support for the project by the Federal Ministry of Education and Research of Germany (BMBF).\\Corresponding author: {\tt\footnotesize lars.ullrich@fau.de}}
	\thanks{\IEEEauthorrefmark{2}Chair of Automatic Control, Friedrich-Alexander-Universität Erlangen-Nürnberg (FAU), Cauerstraße 7, 91058 Erlangen, Germany {\tt\footnotesize \{lars.ullrich, knut.graichen\}@fau.de}}
	\thanks{\IEEEauthorrefmark{3}Institute of Measurement, Control and Microtechnology, Ulm University, Albert-Einstein-Allee 41, 89081 Ulm, Germany {\tt\footnotesize \{michael.buchholz, klaus.dietmayer\}@uni-ulm.de}}}

% The paper headers
\markboth{IEEE Transactions of Intelligent Vehicles, December~2024}%
{Shell \MakeLowercase{\textit{et al.}}: A Sample Article Using IEEEtran.cls for IEEE Journals}


==> settings/packages.tex <==
\usepackage{amsmath,amsfonts,amssymb}
\usepackage{algorithmic}
\usepackage{algorithm}
\usepackage{array}
%\usepackage[caption=false,font=normalsize,labelfont=sf,textfont=sf]{subfig}
\usepackage{textcomp}
\usepackage{stfloats}
\usepackage{url}
\usepackage{verbatim}
\usepackage{graphicx}
\usepackage{subcaption}
\usepackage{cite}

\usepackage{xcolor}
\usepackage{siunitx}
\usepackage{booktabs}


\usepackage{arydshln} % For dashed lines
% Custom dashed midrule command
\newcommand{\dashmidrule}{%
    \noalign{\vskip 0.8ex} % Fine-tune spacing above the dashed line
    \hdashline[2.0pt/2pt] % The dashed line itself
    \noalign{\vskip 0.8ex} % Fine-tune spacing below the dashed line
}

% \usepackage{xcolor}
% \usepackage{pgfplots}
% \usepackage{pgfplotstable}

\usepackage{xurl}
\usepackage{tabularx}
\usepackage{diagbox}
\usepackage{makecell}


% Spacing Adjustment
\addtolength{\textfloatsep}{-0.15 in}
\renewcommand{\baselinestretch}{0.951}
\usepackage{adjustbox}


\usepackage{tikz}
\newcommand{\tikzxmark}{%
	\tikz[scale=0.23] {
		\draw[line width=0.7,line cap=round] (0,0) to [bend left=6] (1,1);
		\draw[line width=0.7,line cap=round] (0.2,0.95) to [bend right=3] (0.8,0.05);
}}
\newcommand{\tikzcmark}{%
	\tikz[scale=0.23] {
		\draw[line width=0.7,line cap=round] (0.25,0) to [bend left=10] (1,1);
		\draw[line width=0.8,line cap=round] (0,0.35) to [bend right=1] (0.23,0);
}}

\usepackage{bbding}
\usepackage{pifont}% http://ctan.org/pkg/pifont
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%
%\usepackage{arevmath}
\usepackage{multirow}


\renewcommand{\theenumi}{\roman{enumi}} % Use lowercase Roman numerals for 

\usepackage{scalerel}
\usepackage{tikz}
\usetikzlibrary{svg.path}

\definecolor{orcidlogocol}{HTML}{A6CE39}
\tikzset{
	orcidlogo/.pic={
		\fill[orcidlogocol] svg{M256,128c0,70.7-57.3,128-128,128C57.3,256,0,198.7,0,128C0,57.3,57.3,0,128,0C198.7,0,256,57.3,256,128z};
		\fill[white] svg{M86.3,186.2H70.9V79.1h15.4v48.4V186.2z}
		svg{M108.9,79.1h41.6c39.6,0,57,28.3,57,53.6c0,27.5-21.5,53.6-56.8,53.6h-41.8V79.1z M124.3,172.4h24.5c34.9,0,42.9-26.5,42.9-39.7c0-21.5-13.7-39.7-43.7-39.7h-23.7V172.4z}
		svg{M88.7,56.8c0,5.5-4.5,10.1-10.1,10.1c-5.6,0-10.1-4.6-10.1-10.1c0-5.6,4.5-10.1,10.1-10.1C84.2,46.7,88.7,51.3,88.7,56.8z};
	}
}

\newcommand\orcidicon[1]{\href{https://orcid.org/#1}{\mbox{\scalerel*{
				\begin{tikzpicture}[yscale=-1,transform shape]
					\pic{orcidlogo};
				\end{tikzpicture}
			}{|}}}}

\usepackage{hyperref} 
\hypersetup{
	bookmarks=false,
	colorlinks=true,
	breaklinks=true,
	linkcolor=blue,
	filecolor=magenta,      
	hypertexnames=true,
	urlcolor=cyan,
	pagebackref=true,
	pdfpagemode=FullScreen,
	citecolor=green
}
\urlstyle{same}




